Weakly synchronous systems with three machines are Turing powerful

Communicating finite-state machines (CFMs) are a Turing powerful model of asynchronous message-passing distributed systems. In weakly synchronous systems, processes communicate through phases in which messages are first sent and then received, for each process. Such systems enjoy a limited form of synchronization, and for some communication models, this restriction is enough to make the reachability problem decidable. In particular, we explore the intriguing case of p2p (FIFO) communication, for which the reachability problem is known to be undecidable for four processes, but decidable for two. We show that the configuration reachability problem for weakly synchronous systems of three processes is undecidable. This result is heavily inspired by our study on the treewidth of the Message Sequence Charts (MSCs) that might be generated by such systems. In this sense, the main contribution of this work is a weakly synchronous system with three processes that generates MSCs of arbitrarily large treewidth.

==> apx-is-ws-p2p.tex <==
We show here that graphs such as that of Fig.\ref{fig:ws_p2p_minor_k3_3} are minors of some weakly synchronous \pp MSC with 1 exchange. The last graph in Fig.\ref{fig:is_ws_p2p} shares the same structure as that of Fig.\ref{fig:ws_p2p_minor_k3_3}, but it is a little simpler for illustration purposes\footnote{In particular, it is a little bit smaller and it misses the left part of the graph in Fig.\ref{fig:ws_p2p_minor_k3_3}, which is already weakly synchronous by construction and does not introduce any additional difficulties.}; let us call this graph $G_1$. Also note that the MSC in the top left of Fig.\ref{fig:is_ws_p2p} is a weakly synchronous \pp MSC with 3 processes; the picture shows that, after some edge contractions, we get $G_1$. Given any graph $G$, such as $G_1$, constructed in the way that was specified in the first part of the proof, it is easy to a weakly synchronous \pp MSC that has $G$ has minor, as shown in Fig.\ref{fig:is_ws_p2p} (just follow the arrows in the inverse order starting from $G_1$). Roughly, we just have to split some nodes in two, since our notion of MSC does not admit that multiple messages are sent or received by a single event\footnote{Note that we can find multiple weakly synchronous MSCs that have G as a minor, since we can choose how to order nodes when we split them.}.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{is_ws_p2p}
    \caption{A graph (bottom right) constructed using the technique presented in the first part of the proof of Prop.\ref{prop:ws_p2p_4_tw} is always a minor of some weakly synchronous \pp MSC (top left) with 1 exchange. The steps show some edge contractions applied to the MSC. Please note that we consider the underlining undirected graph of the MSC in these steps, since we do not care about the orientation of arcs. In step 1, we merge some nodes on the red path. In steps 2 and 3, we do the same for the blue and the green paths.} 
    \label{fig:is_ws_p2p}
\end{figure}	

==> chapters/ch-prelim-graphs.tex <==
There is a strong correlation between MSCs and graphs. An MSC is a directed graph where the nodes are the events of the MSC and the edges are represented by the $\procrel$ and the $\lhd$ relations. We are therefore able to use some tools and techniques from graph theory to possibly derive some interesting results about MSCs.

\begin{definition} 
    A {\it tree-decomposition} of a graph $G=(V,E)$ is a pair $(T, {\cal X}=\{ X_{t}\mid t \in V(T)\})$ such that $T$ is a tree, and ${\cal X}$ is a set of subsets (called {\it bags}) of $V$, one for each node of $T$, such that:

    \begin{itemize}
        \item $\bigcup_{t\in V(T)} X_{t} = V(G)$;
        \item for every $\{u,v\}\in E(G)$, there exists $t \in V(T)$ such that $u, v\in X_{t}$;
        \item for every $v \in V(G)$, the set $\{t \in V(T) \mid v \in X_t\}$ induces a subtree of $T$.
    \end{itemize}

\end{definition}
The {\it width} of a tree decomposition $(T, {\cal X})$ is $\max_{t \in V(T)} |X_t|-1$, i.e., the size of the largest bag minus one. The {\it treewidth} $tw(G)$ of $G$ is the minimum width over all possible tree decompositions of $G$. If $T$ is a path, then we call $(T, {\cal X})$ a \emph{path decomposition} of $G$, and the \emph{pathwidth} $pw(G)$ of $G$ is the minimum width over all possible path decompositions of $G$.

\begin{definition}
    A graph $G$ is a \emph{minor} of a graph $H$, if $G$ can be obtained from $H$ by a series of vertex deletions, edge deletions, and edge contractions, where an edge contraction is the operation that replaces two adjacent vertices $v$ and $w$ by a single vertex that is adjacent to all the neighbors of $v$ and $w$.
\end{definition}

The following well-known result in graph theory gives a connection between the notions of treewidth and minor.

\begin{theorem}[Minor theorem]
\label{thm:minor_tw}
    If $G$ is a minor of $H$, then $tw(G) \le tw(H)$, and $pw(G) \le pw(H)$.
\end{theorem}
